Isotropic MIMO Interference Channels without CSIT: The Loss of Degrees of Freedom

This paper studies two-user MIMO interference channel with isotropic fading. We assume that users are equipped with arbitrary number of antennas and the channel state information (CSI) is available at receivers only. An outer bound is obtained for the degree of freedom region, which suggests the loss of degrees of freedom due to the lack of CSI at transmitters under many circumstances.

==> zycommandset.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{coro}[theorem]{Corollary}
\newtheorem{defi}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{conj}{Conjecture}

\newcommand{\mbA}{\mathbf{A}}
\newcommand{\mbB}{\mathbf{B}}
\newcommand{\mbC}{\mathbf{C}}
\newcommand{\mbD}{\mathbf{D}}
\newcommand{\mbE}{\mathbf{E}}
\newcommand{\mbF}{\mathbf{F}}
\newcommand{\mbG}{\mathbf{G}}
\newcommand{\mbH}{\mathbf{H}}
\newcommand{\mbI}{\mathbf{I}}
\newcommand{\mbJ}{\mathbf{J}}
\newcommand{\mbK}{\mathbf{K}}
\newcommand{\mbL}{\mathbf{L}}
\newcommand{\mbM}{\mathbf{M}}
\newcommand{\mbN}{\mathbf{N}}
\newcommand{\mbO}{\mathbf{O}}
\newcommand{\mbP}{\mathbf{P}}
\newcommand{\mbQ}{\mathbf{Q}}
\newcommand{\mbR}{\mathbf{R}}
\newcommand{\mbS}{\mathbf{S}}
\newcommand{\mbT}{\mathbf{T}}
\newcommand{\mbU}{\mathbf{U}}
\newcommand{\mbV}{\mathbf{V}}
\newcommand{\mbW}{\mathbf{W}}
\newcommand{\mbX}{\mathbf{X}}
\newcommand{\mbY}{\mathbf{Y}}
\newcommand{\mbZ}{\mathbf{Z}}

\newcommand{\mba}{\mathbf{a}}
\newcommand{\mbb}{\mathbf{b}}
\newcommand{\mbc}{\mathbf{c}}
\newcommand{\mbd}{\mathbf{d}}
\newcommand{\mbe}{\mathbf{e}}
\newcommand{\mbf}{\mathbf{f}}
\newcommand{\mbg}{\mathbf{g}}
\newcommand{\mbh}{\mathbf{h}}
\newcommand{\mbi}{\mathbf{i}}
\newcommand{\mbj}{\mathbf{j}}
\newcommand{\mbk}{\mathbf{k}}
\newcommand{\mbl}{\mathbf{l}}
\newcommand{\mbm}{\mathbf{m}}
\newcommand{\mbn}{\mathbf{n}}
\newcommand{\mbo}{\mathbf{o}}
\newcommand{\mbp}{\mathbf{p}}
\newcommand{\mbq}{\mathbf{q}}
\newcommand{\mbr}{\mathbf{r}}
\newcommand{\mbs}{\mathbf{s}}
\newcommand{\mbt}{\mathbf{t}}
\newcommand{\mbu}{\mathbf{u}}
\newcommand{\mbv}{\mathbf{v}}
\newcommand{\mbw}{\mathbf{w}}
\newcommand{\mbx}{\mathbf{x}}
\newcommand{\mby}{\mathbf{y}}
\newcommand{\mbz}{\mathbf{z}}

\newcommand{\ud}{\mathrm{d}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uH}{\mathrm{H}}


\newcommand{\fixme}[1]{{\color{red} #1}}
\newcommand{\modify}[1]{{\color{blue} #1}}
\newcommand{\comment}[1]{{\color{green} #1}}

==> zymacroset.tex <==
\usepackage{ifthen}

\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{coro}[theorem]{Corollary}
\newtheorem{defn}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{conj}{Conjecture}
\newtheorem{claim}{Claim}

\ifthenelse{\equal{\dongningstyle}{true}}{
        \newcommand{\RVEC}[1]{\boldsymbol{\uppercase{#1}}}
        \newcommand{\RMAT}[1]{\underline{\boldsymbol{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\uppercase{#1}}
        \newcommand{\VEC}[1]{\boldsymbol{\lowercase{#1}}}
        \newcommand{\MAT}[1]{\boldsymbol{\underline{\lowercase{#1}}}}
}{
        \newcommand{\RVEC}[1]{\boldsymbol{\lowercase{#1}}}
        \newcommand{\RMAT}[1]{\boldsymbol{\mathrm{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\boldsymbol{\lowercase{#1}}}
        \newcommand{\VEC}[1]{\lowercase{#1}}
        \newcommand{\MAT}[1]{\mathrm{\uppercase{#1}}}
}




\newcommand{\snr}{\mathsf{snr}}
\newcommand{\mmse}{\mathsf{mmse}}
\newcommand{\inr}{\mathsf{INR}}
\newcommand{\MEXP}{\mathbb{E}}
\newcommand{\Prob}[1]{\mathsf{P}\left( #1 \right)}
\newcommand{\Probb}{\mathsf{P}}
\newcommand{\LOG}[1]{\log \left( #1 \right)}
\newcommand{\HAT}[1]{\widehat{#1}}
\newcommand{\TIT}[1]{\widetilde{#1}}
\newcommand{\FLR}[1]{\lfloor #1 \rfloor}
\allowdisplaybreaks

\newcommand{\uT}{\mathsf{T}}
\newcommand{\ud}{\mathsf{d}}
\newcommand{\trace}{\mathsf{tr}}


\newcommand{\fixme}[1]{{\color{Orangered} #1}}
\newcommand{\modify}[1]{{\color{Navyblue} #1}}

